Unifying Function- and Argument-First Bidirectional Type Systems

Bidirectional typing mixes type synthesis and type checking into a single process. Existing bidirectional type systems can be classified into two styles based on whether, given a function application, a bidirectional typing algorithm synthesizes the function's type first and typechecks the argument against the synthesized argument type, or it synthesizes the arguments' types first and typechecks the function against the synthesized arguments' types. We call the former _function-first_ and the latter _argument-first_. Not only do the two styles significantly differ in how the type systems and typing algorithms are formalized, but also they lead to incompatible typeabilities, forcing a language designer to select one style and to give up the other's typeabilities. In this paper, we unify the two styles and develop \lang with a new bidirectional type system for higher-rank polymorphism. Key ideas of the unification are twofold. Each function application is annotated with a bit of information to represent whether function- or argument-first typing is used, to allow a language designer (or even a programmer) to switch between the two styles at their discretion. We reformulate the function- and argument-first type systems by using ideas from colored types and boxy types, which can specify which part of a type should be synthesized or used for checking in a flexible manner. We also develop a typing algorithm based on the worklist approach by Zhao et al. The (declarative) type system of $\lambda^{BH}$ is shown to be sound and to subsume two representative function- and argument-first systems. Our typing algorithm is shown to be sound with respect to the type system of $\lambda^{BH}$ and complete with respect to representative function- and argument-first systems. We mechanically prove the metatheorems using the Abella theorem prover.

==> lang.tex <==
%
\newcommand{\ottdrule}[4][]{{\displaystyle\frac{\begin{array}{l}#2\end{array}}{#3}\quad\ottdrulename{#4}}}
\newcommand{\ottusedrule}[1]{\[#1\]}
\newcommand{\ottpremise}[1]{ #1 \\}
\newenvironment{ottdefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]}{}
\newenvironment{ottfundefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]\begin{displaymath}\begin{array}{l}}{\end{array}\end{displaymath}}
\newcommand{\ottfunclause}[2]{ #1 \equiv #2 \\}
\newcommand{\ottnt}[1]{\mathit{#1}}
\newcommand{\ottmv}[1]{\mathit{#1}}
\newcommand{\ottkw}[1]{\mathbf{#1}}
\newcommand{\ottsym}[1]{#1}
\newcommand{\ottcom}[1]{\text{#1}}
\newcommand{\ottdrulename}[1]{\textsc{#1}}
\newcommand{\ottcomplu}[5]{\overline{#1}^{\,#2\in #3 #4 #5}}
\newcommand{\ottcompu}[3]{\overline{#1}^{\,#2<#3}}
\newcommand{\ottcomp}[2]{\overline{#1}^{\,#2}}
\newcommand{\ottgrammartabular}[1]{\begin{supertabular}{llcllllll}#1\end{supertabular}}
\newcommand{\ottmetavartabular}[1]{\begin{supertabular}{ll}#1\end{supertabular}}
\newcommand{\ottrulehead}[3]{$#1$ & & $#2$ & & & \multicolumn{2}{l}{#3}}
\newcommand{\ottprodline}[6]{& & $#1$ & $#2$ & $#3 #4$ & $#5$ & $#6$}
\newcommand{\ottfirstprodline}[6]{\ottprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\ottlongprodline}[2]{& & $#1$ & \multicolumn{4}{l}{$#2$}}
\newcommand{\ottfirstlongprodline}[2]{\ottlongprodline{#1}{#2}}
\newcommand{\ottbindspecprodline}[6]{\ottprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\ottprodnewline}{\\}
\newcommand{\ottinterrule}{\\[5.0mm]}
\newcommand{\ottafterlastrule}{\\}
%
\renewcommand{\ottkw}[1]{\mathbf{#1} }
\renewcommand{\ottcom}[1]{\textit{#1} }
\renewcommand{\ottcomplu}[5]{#1\mbox{}^{\,#2\in #3 #4 #5} }

\renewcommand{\ottdrulename}[1]{\textsc{#1} }

\newcommand{\ottmetavars}{
\ottmetavartabular{
 $ \ottmv{index} ,\, \ottmv{i} ,\, \ottmv{j} ,\, \ottmv{n} ,\, \ottmv{r} ,\, \ottmv{cont} $ & \ottcom{indices} \\
 $ \ottmv{integer} $ &  \\
 $ \ottmv{char} $ &  \\
 $ \mathit{numvar} $ &  \\
 $ \mathit{termvar} ,\, \mathit{x} ,\, \mathit{y} ,\, \mathit{z} ,\, \mathit{k} ,\, \mathit{f} ,\, \mathit{g} ,\, \mathit{h} $ &  \\
 $ \ottmv{typevar} ,\, \ottmv{a} ,\, \ottmv{b} $ &  \\
 $ \ottmv{mono\_typevar} ,\, \monoalpha ,\, \monobeta ,\, \monogamma $ &  \\
 $ \ottmv{poly\_typevar} ,\, \polyalpha ,\, \polybeta ,\, \polygamma $ &  \\
}}

\newcommand{\otte}{
\ottrulehead{\ottnt{e}  ,\ \ottnt{M}  ,\ \ottnt{N}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottnt{v}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{e_{{\mathrm{1}}}} \, \ottnt{e_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{e_{{\mathrm{1}}}}  \appright  \ottnt{e_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{e_{{\mathrm{1}}}}  \appleft  \ottnt{e_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{e}  \mathbin{@}  \ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{e_{{\mathrm{1}}}}   \mathbin{ \mathit{bop} }   \ottnt{e_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottkw{let} \, \undefined  \ottsym{=}  \ottnt{e_{{\mathrm{1}}}} \, \ottkw{in} \, \ottnt{e_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottnt{e_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{e_{{\mathrm{2}}}}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{e}  \ottsym{:}  \ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottnt{e}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \Lambda  \ottmv{a}  .  \ottnt{e} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{C}  \langle  \ottnt{e}  \rangle }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{e} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ [  \ottnt{v} / \mathit{x}  ]  \ottnt{e} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ [  \ottnt{A} / \ottmv{a}  ]  \ottnt{e} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{e}  \\ & }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \\ &  \ottnt{e} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{e}  \quad }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \quad  \ottnt{e} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ |  \ottnt{e}  | }{}{}{}{}\ottprodnewline
\ottprodline{|}{ |  \ottnt{e}  |_{ \mathrm{DK} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ |  \ottnt{e}  |_{ \mathrm{XO} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ |  \ottnt{e}  |_{ \mathrm{Coer} } }{}{}{}{}}

\newcommand{\ottv}{
\ottrulehead{\ottnt{v}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{x}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\undefined}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \lambda  \undefined  .  \ottnt{e} }{}{}{}{}}

\newcommand{\ottarg}{
\ottrulehead{\undefined}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{x}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathit{x}  \ottsym{:}  \ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \mathit{x}  \ottsym{:}  \ottnt{A}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{()}}{}{}{}{}}

\newcommand{\ottconst}{
\ottrulehead{\undefined  ,\ \ottnt{c}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottsym{()}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \texttt{"}\mathtt{ \ottnt{chars} }\texttt{"} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathit{numvar}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottmv{integer}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathsf{true} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathsf{false} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathsf{id} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ ( \mathbin{ \mathit{bop} } ) }{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathit{uop}}{}{}{}{}}

\newcommand{\ottchars}{
\ottrulehead{\ottnt{chars}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottmv{char}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottmv{char} \  \ottnt{chars} }{}{}{}{}}

\newcommand{\ottbop}{
\ottrulehead{\mathbin{ \mathit{bop} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottsym{+}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{-}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{*}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathbin{/}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathbin{<} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathbin{=} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathbin{ \string^ } }{}{}{}{}}

\newcommand{\ottuop}{
\ottrulehead{\mathit{uop}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \texttt{string\_of\_int} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \texttt{string\_of\_bool} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \texttt{print\_endline} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \texttt{int2str} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \texttt{fst} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \texttt{snd} }{}{}{}{}}

\newcommand{\ottmonoXXtype}{
\ottrulehead{\ottnt{mono\_type}  ,\ \tau  ,\ \sigma}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\iota}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottmv{a}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \tau   \rightarrow   \sigma }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \tau  \times  \sigma }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \tau  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathit{ty}( \ottnt{c} ) }{}{}{}{}\ottprodnewline
\ottprodline{|}{\monoalpha}{}{}{}{}}

\newcommand{\otttype}{
\ottrulehead{\ottnt{type}  ,\ \ottnt{A}  ,\ \ottnt{B}  ,\ \ottnt{S}  ,\ \ottnt{T}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottnt{mono\_type}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathsf{ID} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{A}   \rightarrow   \ottnt{B} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \forall  \ottmv{a}  .  \ottnt{A} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{A}  \times  \ottnt{B} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottnt{A}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ [  \ottnt{A}  /  \ottmv{a}  ]  \ottnt{B} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ [  \ottnt{A}  /  \monoalpha  ]  \ottnt{B} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ |  {A^\Box}  | _ \square }{}{}{}{}\ottprodnewline
\ottprodline{|}{\polyalpha}{}{}{}{}\ottprodnewline
\ottprodline{|}{ - }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \text{?} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \boxed{ \text{?} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathsf{Gen} \, \ottsym{(}  \ottnt{A}  \ottsym{;}  \Gamma  \ottsym{)}}{}{}{}{}}

\newcommand{\ottboxyXXtype}{
\ottrulehead{\ottnt{boxy\_type}  ,\ {A^\Box}  ,\ {B^\Box}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \boxed{ \ottnt{A} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{\iota}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottmv{a}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{A^\Box}  \rightarrow  {B^\Box}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ @  \ottnt{A}   \rightarrow   {B^\Box} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \forall  \ottmv{a}  .  \ottnt{A} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {A^\Box}  \times  {B^\Box} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {A^\Box}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ [  \ottnt{A}  /  \ottmv{a}  ]  {A^\Box} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathsf{ArgChk} ( \Xi ,  \ottnt{A} ) }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathsf{FoldCurry} ( \Xi ,  {A^\Box} ) }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \boxed{ \polyalpha } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ [  \ottnt{A}  /  \monoalpha  ]  {A^\Box} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ [  \ottnt{A}  /  \polyalpha  ]  {A^\Box} }{}{}{}{}}

\newcommand{\ottbaseXXtype}{
\ottrulehead{\undefined  ,\ \iota}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \mathsf{unit} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathsf{int} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathsf{bool} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathsf{str} }{}{}{}{}}

\newcommand{\ottcoercion}{
\ottrulehead{\undefined  ,\ \ottnt{C}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \Diamond^{ \ottnt{A} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{C_{{\mathrm{1}}}}  \rightarrow^{ \ottnt{A} }  \ottnt{C_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \Lambda  \ottmv{a}  .  \ottnt{C} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{C} \, \ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{C_{{\mathrm{1}}}}  \langle  \ottnt{C_{{\mathrm{2}}}}  \rangle }{}{}{}{}}

\newcommand{\ottmark}{
\ottrulehead{\undefined  ,\ \mu}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \text{?} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \text{!} }{}{}{}{}}

\newcommand{\ottmeffect}{
\ottrulehead{\undefined}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \langle  \undefined  ,  \undefined  \rangle }{}{}{}{}}

\newcommand{\ottmtype}{
\ottrulehead{\undefined  ,\ \ottnt{m}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \text{!} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\mu  \rightarrow  \undefined}{}{}{}{}}

\newcommand{\otttypingXXcontext}{
\ottrulehead{\undefined  ,\ \Psi}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \emptyset }{}{}{}{}\ottprodnewline
\ottprodline{|}{\undefined}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi_{{\mathrm{1}}}  \ottsym{,}  \Psi_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \Psi  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ |  \Omega  | }{}{}{}{}}

\newcommand{\ottapplicationXXcontext}{
\ottrulehead{\undefined  ,\ \Xi}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \emptyset }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ @  \ottnt{A} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\Xi_{{\mathrm{1}}}  \ottsym{,}  \Xi_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \Xi  \ottsym{)}}{}{}{}{}}

\newcommand{\ottworkXXlistXXwithoutXXpolytyvars}{
\ottrulehead{\undefined  ,\ \Delta  ,\ \Sigma}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \emptyset }{}{}{}{}\ottprodnewline
\ottprodline{|}{\undefined}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Delta_{{\mathrm{1}}}  \ottsym{,}  \Delta_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Delta  \Vdash  \omega}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Delta_{{\mathrm{1}}}  \ottsym{[}  \Delta_{{\mathrm{2}}}  \ottsym{]}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Delta  \ottsym{[}  \ottsym{]}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ [  \tau  /  \monoalpha  ]  \Delta }{}{}{}{}\ottprodnewline
\ottprodline{|}{ [  \ottnt{A}  /  \polyalpha  ]  \Delta }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \Delta  \ottsym{)}}{}{}{}{}}

\newcommand{\ottworkXXlist}{
\ottrulehead{\undefined  ,\ \Gamma}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \emptyset }{}{}{}{}\ottprodnewline
\ottprodline{|}{\undefined}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Gamma_{{\mathrm{1}}}  \ottsym{,}  \Gamma_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Gamma  \Vdash  \omega}{}{}{}{}\ottprodnewline
\ottprodline{|}{ [  \tau  /  \monoalpha  ]  \Gamma }{}{}{}{}\ottprodnewline
\ottprodline{|}{ [  {A^\Box}  /  \polyalpha  ]  \Gamma }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \Gamma  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \Gamma  \\ }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \Gamma  & }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \Gamma  \quad }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \Gamma  \qquad }{}{}{}{}\ottprodnewline
\ottprodline{|}{\Omega}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Delta}{}{}{}{}}

\newcommand{\ottdworkXXlist}{
\ottrulehead{\undefined  ,\ \Omega}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \emptyset }{}{}{}{}\ottprodnewline
\ottprodline{|}{\undefined}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Omega_{{\mathrm{1}}}  \ottsym{,}  \Omega_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Omega  \Vdash  \omega}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \Omega  \ottsym{)}}{}{}{}{}}

\newcommand{\ottpolyXXtyvars}{
\ottrulehead{\undefined  ,\ \vec{\polyalpha}  ,\ \vec{\polybeta}  ,\ \vec{\polygamma}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\polyalpha}{}{}{}{}\ottprodnewline
\ottprodline{|}{\vec{\polyalpha}  \ottsym{,}  \vec{\polybeta}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ldots }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \vec{\polyalpha}  \ottsym{)}}{}{}{}{}}

\newcommand{\ottbinding}{
\ottrulehead{\undefined}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{x}  \ottsym{:}  \ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottmv{a}}{}{}{}{}}

\newcommand{\ottworkXXbinding}{
\ottrulehead{\undefined}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\undefined}{}{}{}{}\ottprodnewline
\ottprodline{|}{\monoalpha}{}{}{}{}\ottprodnewline
\ottprodline{|}{\polyalpha}{}{}{}{}\ottprodnewline
\ottprodline{|}{\triangleright  \ottsym{\{}  \vec{\polyalpha}  \ottsym{\}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\triangleright  \ottsym{\{}  \ottsym{\}}}{}{}{}{}}

\newcommand{\ottw}{
\ottrulehead{\omega}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottkw{end} \, \ottsym{(}  {A^\Box}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \subL{ \ottnt{A} }{ {B^\Box} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \subR{ {A^\Box} }{ \ottnt{B} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{A}  \mathbin{<:}  \ottnt{B}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{e}  \ottsym{:}  {A^\Box}}{}{}{}{}}

\newcommand{\ottset}{
\ottrulehead{\ottnt{set}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \emptyset }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{set_{{\mathrm{1}}}}   \ottnt{set\_op}   \ottnt{set_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Gamma}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{type\_set}}{}{}{}{}}

\newcommand{\otttypeXXset}{
\ottrulehead{\ottnt{type\_set}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \emptyset }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{\{}  \ottnt{type\_seq}  \ottsym{\}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{\{}  \vec{\polyalpha}  \ottsym{\}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{\{}  \ottsym{\}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{type\_set_{{\mathrm{1}}}}   \ottnt{set\_op}   \ottnt{type\_set_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathrm{FTV}( {A^\Box} ) }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottnt{type\_set}  \ottsym{)}}{}{}{}{}}

\newcommand{\otttypeXXseq}{
\ottrulehead{\ottnt{type\_seq}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{type\_seq}  \ottsym{,}  \ottnt{type}}{}{}{}{}}

\newcommand{\ottsetXXop}{
\ottrulehead{\ottnt{set\_op}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{ \cap }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \cup }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \setminus }{}{}{}{}}

\newcommand{\ottnum}{
\ottrulehead{\ottnt{num}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottmv{integer}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottmv{index}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{num_{{\mathrm{1}}}}  \ottsym{+}  \ottnt{num_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{num_{{\mathrm{1}}}}  \ottsym{-}  \ottnt{num_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \ottnt{num_{{\mathrm{1}}}}  \times  \ottnt{num_{{\mathrm{2}}}} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathsf{size}( \ottnt{e} ) }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \mathsf{msize}( \ottkw{me} ) }{}{}{}{}}

\newcommand{\ottjudgment}{
\ottrulehead{\undefined}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\vdash  \Psi}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi  \vdash  {A^\Box}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi  \vdash  \ottnt{e}  \ottsym{:}  {A^\Box}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \Psi   \vdash  \subL{ \ottnt{A} }{ {B^\Box} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ \Psi   \vdash  \subR{ {A^\Box} }{ \ottnt{B} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{\vdash  \Gamma}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Gamma  \vdash  \ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Gamma  \vdash  {A^\Box}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Gamma  \vdash  \ottnt{e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Gamma  \vdash  \omega}{}{}{}{}\ottprodnewline
\ottprodline{|}{\vdash^\downarrow  \Gamma}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Gamma  \vdash^\downarrow  \ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Gamma  \vdash^\downarrow  {A^\Box}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Gamma  \vdash^\downarrow  \ottnt{e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Gamma  \vdash^\downarrow  \omega}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{type\_set_{{\mathrm{1}}}}  \vdash  \Gamma  \dashv  \ottnt{type\_set_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Gamma  \mid  \ottnt{type\_set_{{\mathrm{1}}}}  \vdash  {A^\Box}  \dashv  \ottnt{type\_set_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Gamma  \mid  \ottnt{type\_set_{{\mathrm{1}}}}  \vdash  \omega  \dashv  \ottnt{type\_set_{{\mathrm{2}}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi  \vdash_{ \mathrm{SysF} }  \ottnt{e}  \ottsym{:}  \ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi  \vdash_{ \mathrm{F}_{\iota} }  \ottnt{e}  \ottsym{:}  \ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi  \vdash_{ \mathrm{F}_{\iota} }  \ottnt{C}  \ottsym{:}  \ottnt{A}  \triangleright  \ottnt{B}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi  \vdash_{ \mathrm{DK} }  \ottnt{A}  \mathbin{<:}  \ottnt{B}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi  \vdash_{ \mathrm{DK} }  \ottnt{e}  \Rightarrow  \ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi  \vdash_{ \mathrm{DK} }  \ottnt{e}  \Leftarrow  \ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ \Psi   \vdash_{ \mathrm{DK} }   \ottnt{A}  \bullet  \ottnt{e}  \Rightarrow\!\!\!\Rightarrow  \ottnt{B} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi  \vdash_{ \mathrm{XO} }  \ottnt{A}  \mathbin{<:}  \ottnt{B}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi  \mid  \Xi  \vdash_{ \mathrm{XO} }  \ottnt{A}  \mathbin{<:}  \ottnt{B}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi  \mid  \Xi  \vdash_{ \mathrm{XO} }  \ottnt{e}  \Rightarrow  \ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi  \vdash  \ottnt{A}  \mathbin{<:}  \ottnt{B}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi  \vdash  \ottnt{e}  \Rightarrow  \ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Psi  \vdash  \ottnt{e}  \Leftarrow  \ottnt{A}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottnt{e_{{\mathrm{1}}}}  \ottsym{:}  \undefined  \twoheadrightarrow  \ottnt{e_{{\mathrm{2}}}}}{}{}{}{}}

\newcommand{\ottgrammar}{\ottgrammartabular{
\otte\ottinterrule
\ottv\ottinterrule
\ottarg\ottinterrule
\ottconst\ottinterrule
\ottchars\ottinterrule
\ottbop\ottinterrule
\ottuop\ottinterrule
\ottmonoXXtype\ottinterrule
\otttype\ottinterrule
\ottboxyXXtype\ottinterrule
\ottbaseXXtype\ottinterrule
\ottcoercion\ottinterrule
\ottmark\ottinterrule
\ottmeffect\ottinterrule
\ottmtype\ottinterrule
\otttypingXXcontext\ottinterrule
\ottapplicationXXcontext\ottinterrule
\ottworkXXlistXXwithoutXXpolytyvars\ottinterrule
\ottworkXXlist\ottinterrule
\ottdworkXXlist\ottinterrule
\ottpolyXXtyvars\ottinterrule
\ottbinding\ottinterrule
\ottworkXXbinding\ottinterrule
\ottw\ottinterrule
\ottset\ottinterrule
\otttypeXXset\ottinterrule
\otttypeXXseq\ottinterrule
\ottsetXXop\ottinterrule
\ottnum\ottinterrule
\ottjudgment\ottafterlastrule
}}

%
\newcommand{\ottdefnss}{
}

\newcommand{\ottall}{\ottmetavars\\[0pt]
\ottgrammar\\[5.0mm]
\ottdefnss}



==> macro.tex <==
\newif\ifmydraft \mydraftfalse
\newif\iftheorem \theoremfalse

\newcommand{\draftcomment}[2]{\ifmydraft{\phantom{}\color{#1}{#2}}\else\ifhmode\unskip\fi\fi\xspace}
\newcommand{\TY}[1]{\draftcomment{red}{TY: #1}}
\newcommand{\TS}[1]{\draftcomment{magenta}{TS: #1}}
\newcommand{\AI}[1]{\draftcomment{orange}{AI: #1}}

\newcommand{\DiffS}{\draftcomment{red}{TY: Diff\textless}}
\newcommand{\DiffE}{\draftcomment{red}{\textgreater}}

\newcommand{\arxiv}[2]{\ifarxiv{\phantom{}{#1}}\else{\phantom{}{#2}}\ifhmode\unskip\fi\fi\xspace}

\newcommand{\tand}{%
  \text{ and }%
}

\newcommand{\tor}{%
  \text{ or }%
}

\newcommand{\tif}{%
  \text{if }%
}

\newcommand{\totherwise}{%
  \text{otherwise}%
}

\newcommand{\twhere}{%
  \text{where }%
}

\newcommand{\tno}{%
  \text{no }%
}

\newcommand{\tst}{%
  \text{ s.t. }
}

\newcommand{\deftitle}[2]{
  \def\tmpa{}\def\tmpb{#2}
  \mbox{}

  \noindent\textbf{#1}
  \ifx\tmpa\tmpb
  \else

    \mbox{}

    \noindent
    #2
  \fi
}

\newcommand{\defeq}{\stackrel{\rm \tiny def}{=}}

\newcommand{\adjustdisplayskip}[1]{%
  \begingroup\abovedisplayskip=3pt\belowdisplayskip=3pt #1\endgroup\ignorespaces%
}

\newcommand{\mycomment}[1]{\relax\ignorespaces}
\newcommand{\todo}[1][]{\textcolor{red}{TODO: #1}}

%
\newcommand{\RRightarrow}{\Rightarrow\!\!\!\Rightarrow}
\newcommand{\appright}{\looparrowright}
\newcommand{\appleft}{\looparrowleft}
\newcommand{\subtypingright}{\ensuremath{\mathbin{\sideset{_\square}{}{\mathop{<:}}}}}
\newcommand{\subtypingleft}{\ensuremath{\mathbin{\sideset{}{_\square}{\mathop{<:}}}}}

\newcommand{\subL}[2]{{#1}\subtypingleft{#2}}
\newcommand{\subR}[2]{{#1}\subtypingright{#2}}

%
\newcommand{\monoalpha}{\alpha}
\newcommand{\monobeta}{\beta}
\newcommand{\monogamma}{\gamma}
%
%
%
\newcommand{\polyalpha}{{\bm{\alpha}}}
\newcommand{\polybeta}{{\bm{\beta}}}
\newcommand{\polygamma}{{\bm{\gamma}}}

%
\newcommand{\lang}{\ensuremath{\lambda^{\mathit{BH}}}\xspace}
\newcommand{\sysfi}{\ensuremath{\text{System F}^p_\iota}\xspace}

%
%
\newcommand{\SLRule}[1]{\textnormal{\scshape SL\texttt{\_}{#1}}\xspace}
%
\newcommand{\SRRule}[1]{\textnormal{\scshape SR\texttt{\_}{#1}}\xspace}
%
\newcommand{\SRBox}{\SRRule{Box}}
\newcommand{\SLBox}{\SLRule{Box}}
\newcommand{\SLUnit}{\SLRule{Unit}}
\newcommand{\SRUnit}{\SRRule{Unit}}
\newcommand{\SLTVar}{\SLRule{TVar}}
\newcommand{\SRTVar}{\SRRule{TVar}}
\newcommand{\SLFun}{\SLRule{Fun}}
\newcommand{\SRFun}{\SRRule{Fun}}
\newcommand{\SLAllR}{\SLRule{$\forall$R}}
\newcommand{\SRAllR}{\SRRule{$\forall$R}}
\newcommand{\SLAllL}{\SLRule{$\forall$L}}
\newcommand{\SRAllL}{\SRRule{$\forall$L}}

%
\newcommand{\TRule}[1]{\textnormal{\scshape T\texttt{\_}{#1}}\xspace}
%
\newcommand{\TUnit}{\TRule{Unit}}
\newcommand{\TVar}{\TRule{Var}}
\newcommand{\TAll}{\TRule{$\forall$}}
\newcommand{\TAbsBox}{\TRule{$\lambda$Box}}
\newcommand{\TAbsFunA}{\TRule{$\lambda$Fun1}}
\newcommand{\TAbsFunB}{\TRule{$\lambda$Fun2}}
\newcommand{\TAAbsBox}{\TRule{$\lambda$:Box}}
\newcommand{\TAAbsFun}{\TRule{$\lambda$:Fun}}
\newcommand{\TAppR}{\TRule{AppR}}
\newcommand{\TAppL}{\TRule{AppL}}

%
%
\newcommand{\ARule}[1]{\textnormal{\scshape A\texttt{\_}{#1}}\xspace}
%
\newcommand{\ATyVar}{\ARule{TVar}}
\newcommand{\AEVar}{\ARule{EVar}}
\newcommand{\ADelim}{\ARule{Delim}}
\newcommand{\AVar}{\ARule{Var}}

%
\newcommand{\ASLRule}[1]{\textnormal{\scshape ASL\texttt{\_}{#1}}\xspace}
%
\newcommand{\ASRRule}[1]{\textnormal{\scshape ASR\texttt{\_}{#1}}\xspace}
%
\newcommand{\ASLBox}{\ASLRule{Box}}
\newcommand{\ASRBox}{\ASRRule{Box}}
\newcommand{\ASLUnit}{\ASLRule{Unit}}
\newcommand{\ASRUnit}{\ASRRule{Unit}}
\newcommand{\ASLTVar}{\ASLRule{TVar}}
\newcommand{\ASRTVar}{\ASRRule{TVar}}
\newcommand{\ASLEVar}{\ASLRule{EVar}}
\newcommand{\ASREVar}{\ASRRule{EVar}}
\newcommand{\ASLFun}{\ASLRule{Fun}}
\newcommand{\ASRFun}{\ASRRule{Fun}}
\newcommand{\ASLAllR}{\ASLRule{$\forall$R}}
\newcommand{\ASRAllR}{\ASRRule{$\forall$R}}
\newcommand{\ASLAllL}{\ASLRule{$\forall$L}}
\newcommand{\ASRAllL}{\ASRRule{$\forall$L}}
%
\newcommand{\ASLExExA}{\ASLRule{ExEx1}}
\newcommand{\ASLExExB}{\ASLRule{ExEx2}}
\newcommand{\ASRExExA}{\ASRRule{ExEx1}}
\newcommand{\ASRExExB}{\ASRRule{ExEx2}}
\newcommand{\ASLExTVarA}{\ASLRule{ExTVar1}}
\newcommand{\ASLExTVarB}{\ASLRule{ExTVar2}}
\newcommand{\ASRExTVarA}{\ASRRule{ExTVar1}}
\newcommand{\ASRExTVarB}{\ASRRule{ExTVar2}}
\newcommand{\ASLExUnitA}{\ASLRule{ExUnit1}}
\newcommand{\ASLExUnitB}{\ASLRule{ExUnit2}}
\newcommand{\ASRExUnitA}{\ASRRule{ExUnit1}}
\newcommand{\ASRExUnitB}{\ASRRule{ExUnit2}}
\newcommand{\ASLExFunA}{\ASLRule{ExFun1}}
\newcommand{\ASLExFunB}{\ASLRule{ExFun2}}
\newcommand{\ASRExFunA}{\ASRRule{ExFun1}}
\newcommand{\ASRExFunB}{\ASRRule{ExFun2}}

%
\newcommand{\ATRule}[1]{\textnormal{\scshape AT\texttt{\_}{#1}}\xspace}
%
\newcommand{\ATUnit}{\ATRule{Unit}}
\newcommand{\ATVar}{\ATRule{Var}}
\newcommand{\ATAll}{\ATRule{$\forall$}}
\newcommand{\ATAbsEx}{\ATRule{$\lambda$Ex}}
\newcommand{\ATAbsBox}{\ATRule{$\lambda$Box}}
\newcommand{\ATAbsFunA}{\ATRule{$\lambda$Fun1}}
\newcommand{\ATAbsFunB}{\ATRule{$\lambda$Fun2}}
\newcommand{\ATAAbsEx}{\ATRule{$\lambda$:Ex}}
\newcommand{\ATAAbsBox}{\ATRule{$\lambda$:Box}}
\newcommand{\ATAAbsFun}{\ATRule{$\lambda$:Fun}}
\newcommand{\ATAppR}{\ATRule{AppR}}
\newcommand{\ATAppL}{\ATRule{AppL}}

%
\newcommand{\InstRule}[1]{\textnormal{\scshape Inst\texttt{\_}{#1}}\xspace}
%
\newcommand{\InstRefl}{\InstRule{Refl}}
\newcommand{\InstEx}{\InstRule{\ensuremath{\monoalpha}}}
\newcommand{\InstNil}{\InstRule{\ensuremath{ \triangleright }}}
\newcommand{\InstPex}{\InstRule{\ensuremath{\polyalpha}}}

%
\newcommand{\MarkRule}[1]{\textnormal{\scshape M\texttt{\_}{#1}}\xspace}
\newcommand{\MUnit}{\MarkRule{Unit}}
\newcommand{\MVar}{\MarkRule{Var}}
\newcommand{\MAbs}{\MarkRule{Abs}}
\newcommand{\MAAbs}{\MarkRule{AAbs}}
\newcommand{\MAppA}{\MarkRule{MApp1}}
\newcommand{\MAppB}{\MarkRule{MApp2}}
\newcommand{\MAppC}{\MarkRule{MApp3}}
\newcommand{\MAppD}{\MarkRule{MApp4}}
\newcommand{\MAppE}{\MarkRule{MApp5}}

